Algorithmic Locality of Quantum Tensor Network Belief Propagation

Belief propagation has recently emerged as a powerful framework for evaluating tensor networks in higher dimensions, combining computational efficiency with provable analytical guarantees. In this work, we develop the first end-to-end theory of tensor network belief propagation for a class of projected entangled pair states satisfying \emph{strong injectivity}. We show that when the injectivity parameter exceeds a constant threshold, BP fixed points can be found efficiently, and a cluster-corrected BP algorithm computes physical quantities to $1/\mathrm{poly}(N)$ error in $\mathrm{poly}(N)$ time for an $N$ qubit system. We further identify a striking phenomenon we term \emph{algorithmic locality}: local perturbations of the tensor network affect the BP fixed point with an influence decaying rapidly with distance. Moreover, through the cluster expansion, this locality extends to observables, implying that local expectation values can be approximated from local data with controlled accuracy. We exhibit three regimes admitting strong injectivity: random Gaussian PEPS with large physical dimension, high-temperature Gibbs states of commuting two-body Hamiltonians, and fixed-depth quantum circuits subject to sufficiently strong depolarizing noise. Our bounds are worst-case sufficient conditions and do not identify sharp algorithmic transitions.

==> tiksstuff.tex <==
% ------------------------------------------------------------------------------------------
% TIKZ
% ------------------------------------------------------------------------------------------
\RequirePackage{tikz}
\usetikzlibrary{decorations.pathreplacing,calligraphy,decorations.markings}
\usetikzlibrary {arrows.meta}

\definecolor{tensorcolor}{rgb}{0.65,0.77,0.95}
\definecolor{btensorcolor}{rgb}{0.65,0.50,0.69}
\definecolor{whitetensorcolor}{rgb}{0.93,0.93,0.93}
% \definecolor{unitary}{rgb}{0.8,0.3,0.3}
\definecolor{gtensorcolor}{rgb}{0.6,0.8,0.5}
\definecolor{operatorcolor}{rgb}{1.0,1.0,1.0}

%\definecolor{unitary}{rgb}{0.8,0.5,.5}
%\definecolor{gate}{rgb}{1.0,1.0,1.0}

%Lengths
\newcommand\doubledx{1.6}
\newcommand\singledx{1.8}
\newcommand\identitydx{1}
\newcommand\stradius{0.6}
\newcommand\unitarydx{2.5}



\newcommand{\GTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=-1
		\draw[very thick] (0,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=1
		\draw[very thick] (-#2,0) -- (0,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (0,#2) -- (0,0);
    \fi

    \ifnum#5=2
		\draw[very thick,draw=red] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=3
		\draw[very thick] (0,-#2) -- (0,#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=4
		\draw[very thick] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=5
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
		\draw[very thick] (0,#2) -- (0,-#2);
    \fi
%
    \ifnum#5=6
		\draw[very thick] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=7
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (0,-#2) -- (0,0);
    \fi
%
    \ifnum#5=8
		\draw[very thick] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=9
		\draw[very thick] (-#2,0) -- (#2,0);
            \draw[very thick] (0,-#2) -- (0,0);
    \fi
        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
		\draw (0,0) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\GFTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (\singledx+#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick, draw=black] (0,#2) -- (0,0);
            \draw[very thick, draw=black] (\singledx,#2) -- (\singledx,0);
    \fi
%
    \ifnum#5=1
		\draw[very thick, draw=red] (-#2,0) -- (\singledx+#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick, draw=black] (0,-#2) -- (0,0);
            \draw[very thick, draw=black] (\singledx,-#2) -- (\singledx,0);
    \fi
%
    \ifnum#5=2
		\draw[very thick, draw=red] (0,-#2) -- (0,#2);
            \draw[very thick, draw=red] (\singledx,-#2) -- (\singledx,#2);
    \fi
%
    \ifnum#5=3
		\draw[very thick] (0,-#2) -- (0,#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=4
		\draw[very thick] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3+\singledx,#3);
		\draw (0+0.5*\singledx,0) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\UFTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		% \draw[very thick, draw=red] (-#2,0) -- (\singledx+#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (\singledx,#2) -- (\singledx,-#2);
    \fi
%
    \ifnum#5=1
		\draw[very thick, draw=red] (0,-#2) -- (0,0);
            \draw[very thick, draw=red] (\singledx,-#2) -- (\singledx,0);
            \draw[very thick] (0.5*\singledx,#2) -- (0.5*\singledx,0);
    \fi

    \ifnum#5=2
		\draw[very thick, draw=red] (0,#2) -- (0,0);
            \draw[very thick, draw=red] (\singledx,#2) -- (\singledx,0);
            \draw[very thick] (0.5*\singledx,-#2) -- (0.5*\singledx,0);
    \fi
%
    \ifnum#5=3
		\draw[very thick, draw=red] (0,#2) -- (0,-#2);
            \draw[very thick, draw=red] (\singledx,#2) -- (\singledx,-#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=4
		\draw[very thick] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
        \draw[ thick, fill=whitetensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3+\singledx,#3);
		\draw (0+0.5*\singledx,0) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\GPTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
            \draw[very thick, draw=red] (0,-#2) -- (0,#2);
    \fi
%
    \ifnum#5=1
		\draw[very thick, draw=red] (-#2,0.2) -- (#2,0.2);
            \draw[very thick, draw=red] (-#2,-0.2) -- (#2,-0.2);
            \draw[very thick, draw=red] (0.2,-#2) -- (0.2,#2);
            \draw[very thick, draw=red] (-0.2,-#2) -- (-0.2,#2);
    \fi

    \ifnum#5=2
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
            \draw[very thick, draw=red] (0,-#2) -- (0,#2);
    \fi

    \ifnum#5=3
		\draw[very thick] (0,-#2) -- (0,#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
	\draw (0,0) node {\scriptsize #4};
    \ifnum#5=0
		\draw[very thick] (#3/2,#3/2) -- (#2,#2);
    \fi
	\end{scope}
}

\newcommand{\UPTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
            \draw[very thick, draw=red] (0,-#2) -- (0,#2);
    \fi
%
    \ifnum#5=1
		\draw[very thick, draw=red] (-#2,0.2) -- (#2,0.2);
            \draw[very thick, draw=red] (-#2,-0.2) -- (#2,-0.2);
            \draw[very thick, draw=red] (0.2,-#2) -- (0.2,#2);
            \draw[very thick, draw=red] (-0.2,-#2) -- (-0.2,#2);
    \fi

    \ifnum#5=2
		\draw[very thick] (-#2,0) -- (#2,0);
            \draw[very thick] (0,-#2) -- (0,#2);
    \fi

    \ifnum#5=3
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
            \draw[very thick, draw=red] (0,-#2) -- (0,#2);
    \fi
%
        \draw[ thick, fill=whitetensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
	\draw (0,0) node {\scriptsize #4};
    \ifnum#5=0
		\draw[very thick] (#3/2,#3/2) -- (#2,#2);
    \fi
    \ifnum#5=2
		\draw[very thick] (#3/2,#3/2) -- (0.75*#2,0.75*#2);
    \fi
    \ifnum#5=3
		\draw[very thick] (#3/2,#3/2) -- (0.75*#2,0.75*#2);
    \fi
	\end{scope}
}

\newcommand{\EPTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0.2) -- (#2,0.2);
            \draw[very thick, draw=red] (-#2,-0.2) -- (#2,-0.2);
            \draw[very thick, draw=red] (0.2,-#2) -- (0.2,#2);
            \draw[very thick, draw=red] (-0.2,-#2) -- (-0.2,#2);
    \fi
%
    \ifnum#5=1
		\draw[very thick, draw=red] (-#2,0.2) -- (#2,0.2);
            \draw[very thick, draw=red] (-#2,-0.2) -- (#2,-0.2);
            \draw[very thick, draw=red] (0.2,-#2) -- (0.2,#2);
            \draw[very thick, draw=red] (-0.2,-#2) -- (-0.2,#2);
    \fi

    \ifnum#5=2
		\draw[very thick,draw=red] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi

    \ifnum#5=3
		\draw[very thick] (0,-#2) -- (0,#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
	\draw (0,0) node {\scriptsize #4};
        % \draw[very thick] (#3/2,#3/2) -- (#2,#2);
	\end{scope}
}

\newcommand{\Unitary}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (-#2,2*#3) -- (#2,2*#3);
    \fi
%
    \ifnum#5=-1
		\draw[very thick] (0,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=1
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick] (0,2*#3) -- (#2,2*#3);
    \fi

    \ifnum#5=2
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            \draw[very thick, draw=red] (-#2,2*#3) -- (#2,2*#3);
    \fi

    \ifnum#5=3
		\draw[very thick] (0,-#2) -- (0,#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,3*#3);
		\draw (0,#3) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\FUnitary}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
            \draw[very thick, draw=red] (-#2,2*#3) -- (#2,2*#3);
            \draw[very thick, draw=red] (-#2,4*#3) -- (#2,4*#3);
    \fi
%
    \ifnum#5=1
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
            \draw[very thick, draw=red] (0,2*#3) -- (#2,2*#3);
            \draw[very thick, draw=red] (0,4*#3) -- (#2,4*#3);
    \fi
%
    \ifnum#5=2
		\draw[very thick,draw=red] (-#2,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi

    \ifnum#5=3
		\draw[very thick] (0,-#2) -- (0,#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,5*#3);
		\draw (0,2*#3) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\PTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw = red] (0,-#2) -- (0,0);
            \draw[very thick, draw = red] (0,0) -- (0,#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=1
		\draw[very thick, draw = red] (-#2,0) -- (0,0);
            \draw[very thick, draw = red] (0,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=2
		\draw[very thick, draw = red] (0,-#2) -- (0,0);
            \draw[very thick, draw = red] (0,0) -- (0,#2);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
    \ifnum#5=3
		\draw[very thick, draw = red] (-#2,0) -- (0,0);
            \draw[very thick, draw = red] (0,0) -- (#2,0);
		% \draw[very thick] (0,#2) -- (0,-#2);
            % \draw[very thick] (0,#2) -- (0,0);
    \fi
%
        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
		\draw (0,0) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\BTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=1
		\draw[very thick,draw=red] (0,#2) -- (0,-#2);
    \fi
%
    \ifnum#5=2
		\draw[very thick] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=3
		\draw[very thick] (0,#2) -- (0,-#2);
    \fi

        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
		\draw (0,0) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\DTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=1
		\draw[very thick,draw=red] (0,#2) -- (0,-#2);
    \fi
%
    \ifnum#5=2
		\draw[very thick] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=3
		\draw[very thick] (0,#2) -- (0,-#2);
    \fi

        \draw[ thick, fill=whitetensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
		\draw (0,0) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\UTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=1
		\draw[very thick,draw=red] (0,#2) -- (0,-#2);
    \fi
%
    \ifnum#5=2
		\draw[very thick] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=3
		\draw[very thick] (0,#2) -- (0,-#2);
    \fi
%
        \draw[ thick, fill=operatorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
		\draw (0,0) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\RTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick, draw=red] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=1
		\draw[very thick,draw=black] (0,#2) -- (0,-#2);
    \fi
%
    \ifnum#5=2
		\draw[very thick] (-#2,0) -- (#2,0);
    \fi
%
    \ifnum#5=3
		\draw[very thick,draw=red] (-#2,0) -- (#2,0);
    \fi
%
        \draw[ thick, fill=white, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
		\draw (0,0) node {\scriptsize #4};
	\end{scope}
}

\newcommand{\GDTensor}[5]{
	\begin{scope}[shift={(#1)}]
%
    \ifnum#5=0
		\draw[very thick] (-#2,0) -- (#2,0);
		\draw[very thick] (0,#2) -- (0,-#2);
    \fi
%
    \ifnum#5=-1
		\draw[very thick] (0,0) -- (#2,0);
		\draw[very thick] (0,#2) -- (0,-#2);
    \fi
%
    \ifnum#5=1
		\draw[very thick] (-#2,0) -- (0,0);
		\draw[very thick] (0,#2) -- (0,-#2);
    \fi
%
        \draw[ thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
    \def\dx{#3/3};
	\draw [thick]  (-#3+\dx, \dx) -- (- \dx,#3-\dx);
	\draw [thick] (-#3+1.5*\dx,-#3+1.5*\dx) -- (#3-1.5*\dx,#3-1.5*\dx);
	\draw [thick]  ( \dx, -#3 + \dx) -- (#3 - \dx,-\dx);
	\draw (0,0) node {\scriptsize #4};
	\end{scope}
}


% A little "vector" = white circle + one leg in a chosen direction.
% Args:
%  #1 = (x,y) shift
%  #2 = leg length (e.g. 0.8)
%  #3 = circle radius (e.g. 0.14)
%  #4 = direction code: 0=right, 1=up, 2=left, 3=down
%  #5 = optional label (can be empty)
\newcommand{\VecCirc}[5]{%
  \begin{scope}[shift={(#1)}]
    \ifnum#4=0 \draw[very thick] (#3,0) -- (#2,0); \fi
    \ifnum#4=1 \draw[very thick] (0,#3) -- (0,#2); \fi
    \ifnum#4=2 \draw[very thick] (-#3,0) -- (-#2,0); \fi
    \ifnum#4=3 \draw[very thick] (0,-#3) -- (0,-#2); \fi
    \draw[very thick, fill=white] (0,0) circle (#3);
    \node at (0,0) {\scriptsize #5};
  \end{scope}%
}



%Modifications
\newcommand\subsetsim{\mathrel{%
  \ooalign{\raise0.2ex\hbox{$\subset$}\cr\hidewidth\raise-0.8ex\hbox{\scalebox{0.9}{$\sim$}}\hidewidth\cr}}}



  % Plain 4-leg tensor: all black, no extra "physical" stub.
% Args:
%  #1 = (x,y) shift
%  #2 = leg half-length (e.g. 1.1)  [legs run from +-#2 to the tensor]
%  #3 = half box size (e.g. 0.45)
%  #4 = label
\newcommand{\PlainTensorFour}[4]{%
  \begin{scope}[shift={(#1)}]
    % four legs (black)
    \draw[very thick] (-#2,0) -- (-#3,0);
    \draw[very thick] ( #3,0) -- ( #2,0);
    \draw[very thick] (0,-#2) -- (0,-#3);
    \draw[very thick] (0, #3) -- (0, #2);
    % square
    \draw[thick, fill=tensorcolor, rounded corners=2pt] (-#3,-#3) rectangle (#3,#3);
    \node at (0,0) {\scriptsize #4};
  \end{scope}%
}

% White circle vector placed at the END of a leg, with a short stub pointing inward.
% Args:
%  #1 = (x,y) shift (this is the circle center, i.e. at the outer endpoint)
%  #2 = stub length toward the tensor (e.g. 0.35)
%  #3 = circle radius (e.g. 0.14)
%  #4 = direction pointing *toward the tensor*: 0=left,1=down,2=right,3=up
%  #5 = optional label (can be empty)
\newcommand{\EndVecCirc}[5]{%
  \begin{scope}[shift={(#1)}]
    \ifnum#4=0 \draw[very thick] (-#3,0) -- (-#2,0); \fi % stub to the left
    \ifnum#4=1 \draw[very thick] (0,-#3) -- (0,-#2); \fi % stub down
    \ifnum#4=2 \draw[very thick] (#3,0) -- (#2,0); \fi % stub right
    \ifnum#4=3 \draw[very thick] (0,#3) -- (0,#2); \fi % stub up
    \draw[very thick, fill=white] (0,0) circle (#3);
    \node at (0,0) {\scriptsize #5};
  \end{scope}%
}

\usetikzlibrary{calc,arrows.meta} % calc for coordinate arithmetic, arrows.meta for Latex tips
\RequirePackage{pgffor} % optional, but makes \foreach definitely available

% Replace edge P--Q by P---o  o---Q
\newcommand{\BPEdge}[4]{%
  \pgfmathsetmacro{\rr}{#3}
  \pgfmathsetmacro{\gg}{#4}
  \pgfmathsetmacro{\dd}{0.5*\gg + \rr} % midpoint-to-center distance

  \coordinate (BPm)  at ($(#1)!0.5!(#2)$);
  \coordinate (BPcL) at ($(BPm)!\dd!(#1)$);
  \coordinate (BPcR) at ($(BPm)!\dd!(#2)$);

  \coordinate (BPpL) at ($(BPcL)!\rr!(#1)$);
  \coordinate (BPpR) at ($(BPcR)!\rr!(#2)$);

  \draw[very thick] (#1) -- (BPpL);
  \draw[very thick] (#2) -- (BPpR);
  \draw[very thick, fill=white] (BPcL) circle (\rr);
  \draw[very thick, fill=white] (BPcR) circle (\rr);
}


\definecolor{opmaroon}{RGB}{120,30,45}



